A Random Forest Approach for Modeling Bounded Outcomes

Random forests have become an established tool for classification and regression, in particular in high-dimensional settings and in the presence of complex predictor-response relationships. For bounded outcome variables restricted to the unit interval, however, classical random forest approaches may severely suffer as they do not account for the heteroscedasticity in the data. A random forest approach is proposed for relating beta distributed outcomes to explanatory variables. The approach explicitly makes use of the likelihood function of the beta distribution for the selection of splits during the tree-building procedure. In each iteration of the tree-building algorithm one chooses the combination of explanatory variable and splitting rule that maximizes the log-likelihood function of the beta distribution with the parameter estimates derived from the nodes of the currently built tree. Several simulation studies demonstrate the properties of the method and compare its performance to classical random forest approaches as well as to parametric regression models.

==> header.tex <==
%% neu 1.9.2011     Abstände zwischen den Einträgen des Literaturverzeichnisses variieren.



%% Schrift
%\usepackage{mathptmx}
%\usepackage[scaled=.90]{helvet}
%\usepackage{courier}



\usepackage{times}      % old but good
%\usepackage{lmodern} %Latex STandard Schrift


%% language, coding
\usepackage[german,english]{babel}
\usepackage[T1]{fontenc}
\usepackage{textcomp}
\usepackage[latin1]{inputenc}

\usepackage{afterpage}

\usepackage{multind}             %multiple Inidices



\usepackage{chicago_new}




\usepackage{amsfonts, amsmath, amssymb, amsthm}
\usepackage{calc}
\usepackage{curves,epic,eepic,latexsym,ifthen}
%new
\usepackage{curves,epic,eepic,amsmath,latexsym,amssymb,array,ifthen,dcolumn}
\usepackage{epsfig}

%new
\usepackage{graphicx}
\usepackage[only,tenrm,svtnrm,egtrm,frtnrm]{rawfonts}

%\usepackage{showkeys}   %Label-Name at margin

\usepackage{rotating}
\usepackage{bbm}

\usepackage{color}
\usepackage{verbatim}
\usepackage{float}
\usepackage{textcomp}
\usepackage[english]{varioref}
\usepackage[scanall]{psfrag}

%Schauberger
\usepackage{tikz}
\usepackage{tikz-qtree}
\usepackage{pgfkeys}

\listfiles

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Tables
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\usepackage{%
  longtable,
  array,
  booktabs,
  dcolumn,
  rotating,
  shortvrb,
  tabularx,
  units,
  multirow
}

%\usepackage{fltpoint}
%\usepackage{rccol}
%\rcDecimalSign{.}


%% booktabs
\setlength{\heavyrulewidth}{0.06em}    % for \toprule and \bottomrule (default 0.08em)
\setlength{\lightrulewidth}{0.04em}    % for \midrulelightrulewidth (default 0.05em)
    % cmidrulewidht = 0.03em (fr \cmidrule)


%% Tables specific letter type
\newenvironment{tabularsmall}
{
\footnotesize \sffamily
\tabular
}
{
\endtabular
\normalfont
}

%% Ausrichtung am Dezimalpunkt
\newcolumntype{d}[1]{D{.}{.}{#1}} %% d{Anz.Dezimalstellen}


\newcolumntype{.}[1]{D{.}{.}{#1}}  %% in count


%% zum leichteren Ausrichten von Tabellenspalten
\newcommand{\ph}[1]{\phantom{#1}}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%         Pages, Margins
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage[
DIVcalc,       % Textbereich (in log-Datei nachlesen)
%DIVclassic
%,headinclude    % dann ist Kopfzeile+Text 18,9cm hoch,
%,headexclude    % dann ist nur der Text 18.9cm hoch + Kopfzeile
%,footexclude    % footinclude
,1.0headlines   %default ist 1.25headlines
%,pagesize
]{typearea}

%\typearea{8}

%\areaset{11.7cm}{18.9cm}
\areaset{13.3cm}{21.0cm}
%kleinerer Abstand von Kopfzeile zu Text
%\setlength{\headheight}{0pt} %13.6pt    holt den Text etwas nï¿½er



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%         fancy head and bottom
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{fancyhdr}

\pagestyle{fancy}
\lhead[\fancyplain{}{\textrm\thepage}]                            % even page
      {\fancyplain{}{\normalfont\footnotesize\scshape\rightmark}} % uneven page
\rhead[\fancyplain{}{\normalfont\footnotesize\scshape\leftmark}]
      {\fancyplain{}{\textrm\thepage}}
\chead{}

\renewcommand{\headrulewidth}{0.5pt} % Trennlinie
\setlength{\headsep}{10pt}           % kleinerer Abstand Text-Kopfzeile (default ist 25pt)

\lfoot{}
\cfoot{\fancyplain{\textrm\thepage}{}}
\rfoot{}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  minipages with boxes
% use  \boxnew[Breite]{Inhalt}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\boxtitle}[1]{\begin{center} \sffamily #1 \end{center}}
\newcommand{\boxitem}[1]{\textsf{\small #1}}

\newcommand{\boxnew}[2][0.8\textwidth]{               %0.8\textwidth als default
   \vspace{1.5ex}          %1ex bewirkt nichts, entspricht 100%
   \begin{center}
   \fbox{%
     \begin{minipage}{#1}   %\linewidth-4ex  ergibt textbreiten Kasten
       {#2}%
     \end{minipage}}%
   \end{center}
   \vspace{2ex}
}

\newcommand{\boxcaption}[1]{
\captionsetup{aboveskip=-1.6ex, belowskip=2ex}
\captionof{table}{#1}
\captionsetup{aboveskip=10pt, belowskip=0pt}
\vspace{1.5ex}
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%         Index (neu 6.7.06 von J.Brandt)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\sindex}[1]{\index{subjectindex}{#1}}
\newcommand{\aindex}[1]{\index{authorindex}{#1}}

% Zweispaltiger Index
\makeatletter
\renewcommand{\printindex}[2]{
   \@restonecoltrue\if@twocolumn\@restonecolfalse\fi
   \columnseprule \z@ \columnsep 35pt   %%obsolet, besser \setlength
   \newpage
   \@mkboth{\MakeUppercase{#2}}{\MakeUppercase{#2}}      %Fr Kopfzeile
%    \twocolumn[{\rm\huge\sffamily\mdseries #2 \vskip4ex}]      %%obsolet, wegen \rm
    \twocolumn[{\rm\huge\sffamily\mdseries #2 \vskip4ex}]
   \addcontentsline{toc}{chapter}{#2}                    %Eintrag ins Inhaltsverzeichnis
   \@input{#1.ind}
 }
\makeatother


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%         Examples including counter
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\makeatletter
\newcommand{\ecaption}[1]{\addcontentsline{loe}{example}{\protect\numberline{\theexample}#1}} %loe: listOfExamples
\newcommand{\l@example}{\@dottedtocline{1}{0em}{3.2em}}

\newcommand{\listofexamples}{
     \chapter*{List of Examples}                  %ï¿½berschrift der Beispielsliste
     \@mkboth{List of Examples}{List of Examples}         %header
%   \addcontentsline{toc}{section}{List of Examples}    %hier liegt das Problem mit den minitocs => statt chapter nun section und es funktioniert
\addcontentsline{toc}{chapter}{List of Examples}
%     \thispagestyle{empty}
     { \@starttoc{loe}}
}
\makeatother

\newcounter{example}[chapter]
\renewcommand{\theexample}{\thechapter.\arabic{example}}

\newenvironment{example}[1]
    {\refstepcounter{example}
     \ecaption{#1}
     \bigskip
     \noindent{\small \sffamily Example \theexample: #1}
     %\noindent{\small \scshape Example \normalfont \theexample: #1}
                    % Schrift der Beispielsberschrift
     \small         % Schrift des Textes (ohne ï¿½berschrift)
     \\}
    {\qed \bigskip}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%         Chapter headings
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\makeatletter
%% aus book.cls kopiert und modifiziert
\renewcommand\chapter{\if@openright\cleardoublepage\else\clearpage\fi
                    \thispagestyle{plain}%
                    \global\@topnum\z@
                    \@afterindentfalse
                    \secdef\@chapter\@schapter}
\def\@chapter[#1]#2{\ifnum \c@secnumdepth >\m@ne
                       \if@mainmatter
                         \refstepcounter{chapter}%
                         \typeout{\@chapapp\space\thechapter.}%
                         \addcontentsline{toc}{chapter}%
                                   {\protect\numberline{\thechapter}#1}%
                       \else
                         \addcontentsline{toc}{chapter}{#1}%
                       \fi
                    \else
                      \addcontentsline{toc}{chapter}{#1}%
                    \fi
                    \chaptermark{#1}%
                    \addtocontents{lof}{\protect\addvspace{10\p@}}%
                    \addtocontents{lot}{\protect\addvspace{10\p@}}%
                    \if@twocolumn
                      \@topnewpage[\@makechapterhead{#2}]%
                    \else
                      \@makechapterhead{#2}%
                      \@afterheading
                    \fi}
\def\@makechapterhead#1{%
  \vspace*{50\p@}%
  {\parindent \z@ \raggedright \sffamily  %\normalfont default, jetzt \sffamily
    \ifnum \c@secnumdepth >\m@ne
      \if@mainmatter
        \huge \@chapapp\space \thechapter %\bfseries  %nur fï¿½r das Wort Chapter
        \par\nobreak
        \vskip 20\p@        %20
      \fi
    \fi
    \interlinepenalty\@M
%    \Huge  #1\par\nobreak  %\bfseries       %fï¿½r die eigentliche ï¿½berschrift
    \huge  #1\par\nobreak  %\bfseries
    \vskip 40\p@        %40
  }}
\def\@schapter#1{\if@twocolumn
                   \@topnewpage[\@makeschapterhead{#1}]%
                 \else
                   \@makeschapterhead{#1}%
                   \@afterheading
                 \fi}
\def\@makeschapterhead#1{           %verï¿½ndert die Schrift der ï¿½berschrift des Inhalts-, Beispiels- und Literaturverzeichnisses
  \vspace*{50\p@}%
  {\parindent \z@ \raggedright
    \sffamily                       %\normalfont alt
    \interlinepenalty\@M
%    \Huge   #1\par\nobreak          %\bfseries
    \huge   #1\par\nobreak
    \vskip 40\p@
  }}
%%

\renewcommand\section{\@startsection {section}{1}{\z@}%
                                   {-3.5ex \@plus -1ex \@minus -.2ex}% Abstand drï¿½ber
                                   {1.1ex \@plus.1ex}      % Abstand drunter
                                   {\sffamily\Large}}
\renewcommand\subsection{\@startsection{subsection}{2}{\z@}%
                                     {-3.25ex\@plus -1ex \@minus -.2ex}%
                                     {1.0ex \@plus .1ex}%
                                     {\sffamily\large}}
\renewcommand\subsubsection{\@startsection{subsubsection}{3}{\z@}%
                                     {-3.25ex\@plus -1ex \@minus -.2ex}%
                                     {0.5ex \@plus .1ex}%
                                     {\sffamily\normalsize}}
\renewcommand\paragraph{\@startsection{paragraph}{4}{\z@}%
                                    {3.25ex \@plus1ex \@minus.2ex}%
                                    {1ex}%
                                    {\sffamily\normalsize}}
\makeatother

%default-Werte
% \newcommand\section{\@startsection {section}{1}{\z@}%
%                                    {-3.5ex \@plus -1ex \@minus -.2ex}%
%                                    {2.3ex \@plus.2ex}%
%                                    {\normalfont\Large\bfseries}}
% \newcommand\subsection{\@startsection{subsection}{2}{\z@}%
%                                      {-3.25ex\@plus -1ex \@minus -.2ex}%
%                                      {1.5ex \@plus .2ex}%
%                                      {\normalfont\large\bfseries}}
% \newcommand\subsubsection{\@startsection{subsubsection}{3}{\z@}%
%                                      {-3.25ex\@plus -1ex \@minus -.2ex}%
%                                      {1.5ex \@plus .2ex}%
%                                      {\normalfont\normalsize\bfseries}}
% \newcommand\paragraph{\@startsection{paragraph}{4}{\z@}%
%                                     {3.25ex \@plus1ex \@minus.2ex}%
%                                     {-1em}%
%                                     {\normalfont\normalsize\bfseries}}
% \newcommand\subparagraph{\@startsection{subparagraph}{5}{\parindent}%
%                                        {3.25ex \@plus1ex \@minus .2ex}%
%                                        {-1em}%
%                                       {\normalfont\normalsize\bfseries}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Im Anhang bekommen chapter, section und subsection wieder andere Bedeutung
% (noch nicht berarbeitet)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \makeatletter
%   \renewcommand*\l@chapter[2]{%
%     \ifnum \c@tocdepth >\m@ne
%       \addpenalty{-\@highpenalty}%
%       \vskip 1.0em \@plus\p@
%       \setlength\@tempdima{1.5em}%
%       \begingroup
%         \parindent \z@ \rightskip \@pnumwidth
%         \parfillskip -\@pnumwidth
%         \leavevmode \bfseries %\mdseries %\sffamily
%         \advance\leftskip\@tempdima
%         \hskip -\leftskip
%         #1\nobreak\hfil \nobreak\hb@xt@\@pnumwidth{\hss #2}\par
%         \penalty\@highpenalty
%       \endgroup
%     \fi}
% \renewcommand{\appendixname}{Appendix}
% \renewcommand{\appendix}{%
%   \setcounter{chapter}{0}
%   \renewcommand{\thechapter}{\Alph{chapter}}%
%   \renewcommand{\chapter}[1]{%
%     \cleardoublepage\thispagestyle{plain}%
%     \refstepcounter{chapter}%
%     \addcontentsline{toc}{chapter}%
%       {%\protect\sffamily%
%        \protect\numberline{\protect\bfseries\protect%   %%dazw.\bfseries
%        \protect\appendixname\protect\hspace{1ex}\thechapter:}\protect\hspace{9ex}\protect##1}%
%     \@mkboth{\MakeUppercase{\appendixname\ \thechapter:\ ##1}}%
%             {\MakeUppercase{\appendixname\ \thechapter:\ ##1}}%
%     {\flushleft\LARGE\mdseries\sffamily%
%      \appendixname\ \thechapter:\ \nohyphens##1\par}%
%   %\chaptermark{##1}\vspace{\baselineskip}
%   }
%   \renewcommand{\section}[1]{
%     \refstepcounter{section}%
%     \addcontentsline{toc}{section}%
%       {%\protect\sffamily%
%        \protect\numberline{\thesection}##1}%
%     {\noindent\large\mdseries\sffamily\thesection~##1\par}
% %    {\flushleft\large\mdseries\sffamily\thesection~##1\par} ohne Trennungen
%   }
%   \renewcommand{\subsection}[1]{
%     \refstepcounter{subsection}%
%     \addcontentsline{toc}{subsection}%
%       {%\protect\sffamily%
%        \protect\numberline{\thesubsection}##1}%
%     {\noindent\normalsize\mdseries\sffamily\thesubsection~##1\par}
% %    {\flushleft\normalsize\mdseries\sffamily\thesubsection~##1\par} ohne Trennungen
%   }
% }
%% \makeatother


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%   Captions
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{caption}[2003/12/20]
\captionsetup{width=\linewidth-2cm,font=footnotesize,labelfont={sc}}
    %font: Einstellung fï¿½r die gesamte Unterschrift
    %labelfont: Einstellung fï¿½r den Bezeichner (``Table'')


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%         Literature  - neu 1.9.2011 JB
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% aus book.cls %%

\makeatletter

\renewenvironment{thebibliography}[1]
     {\chapter*{\bibname}%
      \@mkboth{\MakeUppercase\bibname}{\MakeUppercase\bibname}%
      %     {\rm\Large\sffamily\mdseries \bibname\vskip2ex}     %ergänzt
    \addcontentsline{toc}{chapter}{\bibname}    %ergänzt
      \list{\@biblabel{\@arabic\c@enumiv}}%
           {\settowidth\labelwidth{\@biblabel{#1}}%
            \leftmargin\labelwidth
            \advance\leftmargin\labelsep
            \@openbib@code
            \usecounter{enumiv}%
            \let\p@enumiv\@empty
            \renewcommand\theenumiv{\@arabic\c@enumiv}}%
      \sloppy
      \clubpenalty4000
      \@clubpenalty \clubpenalty
      \widowpenalty4000%
      \sfcode`\.\@m}
     {\def\@noitemerr
       {\@latex@warning{Empty `thebibliography' environment}}%
      \endlist}

\makeatother

\let\oldbibliography\thebibliography
\renewcommand{\thebibliography}[1]{%
\oldbibliography{#1}%
%\setlength{\itemsep}{0ex}           %% Abstand zwischen den Einträgen %%
\setlength{\itemsep}{-0.3ex} }




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%         minitocs: kleine Inhaltsverzeichnisse
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{minitoc}       % kleine Inhaltsverzeichnisse
\setlength{\fboxsep}{1em}  % \fboxsep4mm    %Vergleiche Einstellungen fï¿½r \boxnew
\setlength{\mtcindent}{4pt}
\renewcommand{\mtcfont}{\small\mdseries\sffamily}
\renewcommand{\mtcSfont}{\small\mdseries\sffamily}
\renewcommand{\mtcSSfont}{\small\mdseries\sffamily}

\newcommand{\makeminitoc}{%
\setcounter{minitocdepth}{3}    % Anzahl Gliederungsebenen
   \vspace{3mm}
   \hrule
   \bigskip
   \noindent


%   \fbox{%
   \begin{minipage}{\linewidth -5ex}
     \vspace*{-3ex}
     \nomtcrule
     \minitoc
\hrule
\bigskip
%     \vspace*{-5ex}%3
   \end{minipage}
%   }
\\[3mm]}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%          Applications   ** neu 21.10.09 JB
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% ZÃ¤hler fÃ¼r die Applications innerhalb der Umgebung
\newcounter{application}[chapter]
\renewcommand{\theapplication}{\thechapter.\arabic{application}}

%% Definition der Umgebung 'application'
\newenvironment{application}
    {\refstepcounter{application}
     \bigskip
     \noindent{\small \sffamily Application \theapplication:} % Ãberschrift
     \\
     \small         % Schrift des Textes (ohne Ueberschrift)
     }

    { \bigskip}

%% Fuer leichtere (a), (b), (c) AufzÃ¤hlungen
\usepackage{enumitem}

\newenvironment{abcitemize}
    {\begin{enumerate}[label=(\alph*)]}
    {\end{enumerate}}


% \newenvironment{anwendung}[1]
%     {\refstepcounter{application}
%      \bigskip
%      \noindent{\small \sffamily Application \theapplication:} % Ãberschrift
%      \small         % Schrift des Textes (ohne Ueberschrift)
%      \\
%      #1
%      \begin{enumerate}[label=(\alph*)]
%      }
%     { \end{enumerate} \bigskip}







% %% Variante 2 *****************************************************************

%
%
% \renewcommand{\labelenumi}{\small \textsf{Application \theenumi :}}
%
%
% \newenvironment{anwendungen}%[Ã]
% {\small \begin{enumerate}[leftmargin=*, style=nextline] }
% {\end{enumerate} }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%          Exercises   ** neu 19.11.09 JB
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% ZÃ¤hler fÃ¼r die Exercieses
\newcounter{exercise}[chapter]
\renewcommand{\theexercise}{\thechapter.\arabic{exercise}}

%% Definition der Umgebung 'exercise'
\newenvironment{exercise}
    {\refstepcounter{exercise}
     \bigskip \small
     \noindent \theexercise
     }

    { \bigskip}

